Human Centred Object Co-Segmentation

Co-segmentation is the automatic extraction of the common semantic regions given a set of images. Different from previous approaches mainly based on object visuals, in this paper, we propose a human centred object co-segmentation approach, which uses the human as another strong evidence. In order to discover the rich internal structure of the objects reflecting their human-object interactions and visual similarities, we propose an unsupervised fully connected CRF auto-encoder incorporating the rich object features and a novel human-object interaction representation. We propose an efficient learning and inference algorithm to allow the full connectivity of the CRF with the auto-encoder, that establishes pairwise relations on all pairs of the object proposals in the dataset. Moreover, the auto-encoder learns the parameters from the data itself rather than supervised learning or manually assigned parameters in the conventional CRF. In the extensive experiments on four datasets, we show that our approach is able to extract the common objects more accurately than the state-of-the-art co-segmentation algorithms.

==> hofea.tex <==
% !TEX root = hcoseg.tex




\section{Visual Features}\label{sec:hofea}
\subsection{Human-Object Interaction Feature}

Unlike conventional co-segmentation approaches, we add an important information $\---$ human, to improve the mining ability. As human detection technique has been improved significantly by using more accurate sensors such as Microsoft Kinect\footnote{\url{http://www.microsoft.com/en-us/kinectforwindows/develop/}}, it has become easier to get human information especially in 3D space from images. In our work, we assume the human body has been detected using the existing human detectors. In this section, we introduce a human-object interaction feature in 3D space based on tracked human skeletons by the Kinect sensor. %which provides 3D coordinates of $25$ tracked joints in 3D point cloud. 

Kinect tracked the joints of a human body as in Figure~\ref{fig:hoif}-(a). We focus on modeling physical interactions between the human and the object, such as sitting on the chair, opening the fridge, \etc, which helps detect those objects used by humans in the scene. We model the spatial relationships between objects and different body parts of the human using a histogram of object points lying in the bins surrounding human body parts. We illustrate the feature representation in Figure~\ref{fig:hoif}. 

We first divide the cylinder surrounding the body part into bins. As in Figure~\ref{fig:fea_3d}, we are given the 3D coordinate of each joint of a tracked human after converting the depth image into the 3D point cloud. Each human body parts is represented as a vector starting from a joint to its neighboring joint. Then we divide the cylinder surrounding the body part vector into $15$ bins by segmenting the body part vertically into $3$ parts and the circle surrounding the body part into $5$ regions evenly. Given the point cloud in an object proposal region, we calculate the histogram of the points in these $15$ bins and normalize it by the number of the total points in the object proposal as the final feature $h_i$ (shown a histogram of the body part \emph{spin-base} to \emph{spin-mid} relative to the chair in Figure~\ref{fig:fea_hist}). For multiple people in the scene, we compute the max of the histograms of all humans.
 
The histogram feature captures the distributions of the object points related to the human body in 3D space. It can represent the relative position, size between the humans and objects as well as the human poses and object shapes. For example in Figure~\ref{fig:hoif}, we plot the histogram feature of the body part \emph{spin-base} to \emph{spin-mid} relative to the chair. We can see that the distribution reflects the shape of the chair in the way: the points of the chair-back lie in the distant bins of the upper part, and from the chair-back to the chair-base, points become evenly distributed from the middle part to the lower part. In the experiments in Section~\ref{sec:expdis}, we show that our human-object interaction feature based object clustering gives an ideal accuracy, which can provide a strong relevance of common objects in our CRF model.
 
%\todo{improve analysis}Note that the feature captures the distributions of object points related to the human body. We illustrate the point distribution of two \emph{fridges} and two \emph{microwaves} in Figure~\ref{fig:hfea}. We can see that the distributions of the histograms are similar for the same object class, even though the view perspective and background scene are different. But for different objects, the histograms are totally different. The feature of \emph{fridge} is dense and evenly distributed since it is parallel to the human body, while the feature of \emph{microwave} is sparse and concentrated in certain bins.  We also run an object clustering experiment to evaluate our human features quantitatively on a human action key frame dataset, which will be introduced in detail in Section~\ref{sec:exp}. The results in Table.~\ref{tb:ohre} shows that our feature based clustering provides an ideal purity of the cluster, which can give a strong relevance of common objects in our CRF model.


\begin{figure*}[t]
  \begin{center}
  \subfigure[]{
  \includegraphics[height=2.05cm]{fig/hfea/fea_rgb.png}
  }\hspace{-0.05in}
  \subfigure[]{
  \includegraphics[height=2.05cm]{fig/hfea/fea_3d.png}\label{fig:fea_3d}
  }\hspace{-0.1in}
   \subfigure[]{
  \includegraphics[height=2.4cm]{fig/hfea/fea.png}\label{fig:fea_hist}
  }
  \caption{Our 3D human-object interaction feature. In (a), we are given the joints (green dots) of the tracked human, and a object proposal region (green mask). In (b), we divide the cylinder surrounding each body part vector (red line, \emph{spin-base} to \emph{spin-mid} in the example) into $15$ bins by segmenting the body part vertically into $3$ parts and the circle surrounding the body part into $5$ regions. In (c), we compute the histogram of the points in these $15$ bins and normalize it by the number of the total points in the object proposal.}
   \label{fig:hoif}
 \end{center}
\vspace{-0.2in}
\end{figure*}
\subsection{Object Features}
We use six kernel descriptors~\cite{Bo_NIPS_2010} on both RGB, depth and point cloud of an image as the object features $f_i$: gradient, color, local binary pattern, depth gradient, spin, surface normals, and KPCA/self-similarity, which have been proven to be useful features for RGB-D scene labeling~\cite{Wu_RSS_2014}.


\if 0
\begin{figure*}[t]
  \begin{center}
  \includegraphics[height=2.4cm]{fig/fridge1.png}
  \includegraphics[height=2.4cm]{fig/fridge1_hist.png}
  \includegraphics[height=2.4cm]{fig/fridge2.png}
  \includegraphics[height=2.4cm]{fig/fridge2_hist.png}
  \includegraphics[height=2.4cm]{fig/oven2.png}
  \includegraphics[height=2.4cm]{fig/oven2_hist.png}
  \includegraphics[height=2.4cm]{fig/oven1.png}
  \includegraphics[height=2.4cm]{fig/oven1_hist.png}
  \caption{Illustration of human-object features for \emph{fridge} and \emph{microwave}. The feature of fridge is dense and evenly distributed since it is parallel to the human body, while the feature of microwave is sparse and concentrated in certain bins. We use $18$ human parts from $1$ to $18$ are: Head-Neck, Neck-SpineShoulder, SpineShoulder-SpineMid, SpineMid-SpineBase, SpineShoulder-ShoulderRight, ShoulderRight-ElbowRight, ElbowRight-WristRight, WristRight-HandRight, SpineShoulder-ShoulderLeft, ShoulderLeft-ElbowLeft, ElbowLeft-WristLeft, WristLeft-HandLeft, SpineBase-HipRight, HipRight-KneeRight, KneeRight-AnkleRight, SpineBase-HipLeft, HipLeft-KneeLeft, KneeLeft-AnkleLeft.}
   \label{fig:hfea}
 \end{center}
\vspace{-0.15in}
\end{figure*}
\fi

==> space_saver.tex <==
% Some illegal space-saving macros
% \parskip=1pt
  \abovedisplayskip 3.0pt plus2pt minus2pt%
 \belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{0.98}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}
{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newlength\savedwidth
\newcommand\whline[1]{\noalign{\global\savedwidth\arrayrulewidth
                               \global\arrayrulewidth #1} %
                      \hline
                      \noalign{\global\arrayrulewidth\savedwidth}}
\renewcommand\multirowsetup{\centering}

\newlength{\sectionReduceTop}
\newlength{\sectionReduceBot}
\newlength{\subsectionReduceTop}
\newlength{\subsectionReduceBot}
\newlength{\abstractReduceTop}
\newlength{\abstractReduceBot}
\newlength{\captionReduceTop}
\newlength{\captionReduceBot}
%\newlength{\nameReduceTop}
\newlength{\subsubsectionReduceTop}
\newlength{\subsubsectionReduceBot}
\newlength{\headerReduceTop}
% Negative space for figures set at the bottom of a block of figs
\newlength{\figureReduceBot}

\newlength{\horSkip}
\newlength{\verSkip}

\newlength{\equationReduceTop}

\newlength{\figureHeight}
\setlength{\figureHeight}{1.7in}

%\newlength{\figureFraction}
\setlength{\horSkip}{-.09in}
\setlength{\verSkip}{-.1in}
%\setlength{\figureFraction}{.195}

% figureReduceBot is for figures which are set above text, since latex
% likes putting a lot of space under those
\setlength{\figureReduceBot}{-0.15in}
\setlength{\headerReduceTop}{0in}
%
%\setlength{\subsectionReduceTop}{-0.08in}
%\setlength{\subsectionReduceBot}{-0.05in}
\setlength{\subsectionReduceTop}{-0.02in}
\setlength{\subsectionReduceBot}{-0.02in}
%\setlength{\sectionReduceTop}{-0.03in}
%\setlength{\sectionReduceBot}{-0.03in}
\setlength{\sectionReduceTop}{-0.02in}
\setlength{\sectionReduceBot}{-0.01in}
\setlength{\subsubsectionReduceTop}{-0.06in}
\setlength{\subsubsectionReduceBot}{-0.05in}
%
%
%\setlength{\figureHeight}{1.5in}
\setlength{\abstractReduceTop}{-0.05in}
\setlength{\abstractReduceBot}{-0.10in}
%
%

\setlength{\equationReduceTop}{-0.1in}

%\setlength{\nameReduceTop}{-0.05in}


\setlength{\captionReduceTop}{-0.06in}
\setlength{\captionReduceBot}{-0.07in}

